Bounded verification of message-passing concurrency in Go using Promela and Spin

This paper describes a static verification framework for the message-passing fragment of the Go programming language. Our framework extracts models that over-approximate the message-passing behaviour of a program. These models, or behavioural types, are encoded in Promela, hence can be efficiently verified with Spin. We improve on previous works by verifying programs that include communication-related parameters that are unknown at compile-time, i.e., programs that spawn a parameterised number of threads or that create channels with a parameterised capacity. These programs are checked via a bounded verification approach with bounds provided by the user.

==> eptcsdata.tex <==
\providecommand{\firstpage}{34}
\providecommand{\publicationstatus}{S. Balzer, L. Padovani (Eds.): Programming Language Approaches\\
to Concurrency- \& Communication-cEntric Software (PLACES 2020)\\
EPTCS 314, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.314.4}{10.4204/EPTCS.314.4}}
\pdfoutput=1

